The Red Queen G\"odel Machine: Co-Evolving Agents and Their Evaluators

Self-improving agents are state-of-the-art on agentic coding benchmarks, yet their search methods assume a stationary evaluation criterion. This ignores a central feature of evolution: species adapt as their environments change with them. We introduce the Red Queen G\"odel Machine (RQGM), an evolutionary framework for recursive self-improvement under non-stationary utilities. This allows learned evaluators to improve alongside the agents they guide. On DeepSWE, the RQGM improves over its fixed-evaluator baseline by adding a complementary agent-as-a-judge code-review signal: a co-evolved reviewer grades coder patches to guide search. At low reasoning effort, the RQGM coder passes 82.1% of held-out tasks against the baseline's 75.0%, and nearly matches the GPT-6 Astra model at high effort. In scientific paper writing and reviewing, and Olympiad-level proof writing and grading, co-evolved evaluators provide an evaluation criterion. Anchored to human IMO grades, a co-evolved grader writes its own milestone rubric and exceeds static baselines at a 3x lower search cost, driving the prover to the best mean score. Since the RQGM can modify the search objective across epochs, it can regularize the search. For example, the RQGM reduces self-preference bias via an additional adversarial objective to discover reviewers equally stringent on AI and human work. Guided by these calibrated reviewers, co-evolved writers reach 1.78x-1.86x higher acceptance rates than the baseline under an agent-as-a-judge panel. The RQGM enables self-improving systems where agents and evaluators recursively bootstrap each other beyond static evaluation.

==> preamble/format.tex <==
\makeatletter

\newif\ifpaper@neurips
\newif\ifpaper@mlsys
\newif\ifpaper@twocolumn
\newif\ifpapericlr \newif\ifpaperanon 
\def\paper@@neurips{neurips}
\def\paper@@iclr{iclr}
\def\paper@@arxiv{arxiv}
\ifx\paper@format\paper@@neurips
  \paper@neuripstrue
  \PassOptionsToPackage{numbers,sort&compress}{natbib}\RequirePackage[preprint]{neurips_2026}\renewcommand{\@notice}{}\def\paperbibstyle{unsrtnat}\else
  \ifx\paper@format\paper@@iclr\papericlrtrue\paperanontrue\fi
  \ifx\paper@format\paper@@arxiv\papericlrtrue\fi
  \ifpapericlr
    \let\paper@contentsline\addcontentsline
    \ifpaperanon\else\PassOptionsToPackage{numbers,sort&compress}{natbib}\fi
    \RequirePackage{iclr2027_conference}\let\addcontentsline\paper@contentsline
    \ifpaperanon
      \def\paper@logos{none}\def\paperbibstyle{iclr2027_conference}\else
      \iclrfinalcopy
      \setcitestyle{numbers,square,citesep={,}}\def\paperbibstyle{unsrtnat}\fi
  \else
    \ClassError{paper}{Unknown format `\paper@format'; expected neurips, iclr, or arxiv}{}\fi
\fi

\makeatother


==> preamble/macros.tex <==
\makeatletter

\graphicspath{{figures/}{figures/plots/}{figures/diagrams/}{figures/tikz/}{branding/}}

\newenvironment{widefigure}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{figure*}[#1]\else \@nameuse{figure}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endfigure*}\else \@nameuse{endfigure}\fi}
\newenvironment{widetable}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{table*}[#1]\else \@nameuse{table}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endtable*}\else \@nameuse{endtable}\fi}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\etal}{et~al.\xspace}
\newcommand{\dashes}{---\xspace}

\newcommand{\todo}[1]{{\normalfont\color{red}\,[TODO: #1]\,}}
\newcommand{\note}[2]{{\normalfont\color{blue}\,[#1: #2]}}



\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}


\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} 
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\crefname{theorem}{Thm.}{Thms.}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lem.}{Lems.}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Cor.}{Cors.}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Def.}{Defs.}
\Crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Asm.}{Asms.}
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{proposition}{Prop.}{Props.}
\Crefname{proposition}{Proposition}{Propositions}
\crefname{remark}{Rem.}{Rems.}
\Crefname{remark}{Remark}{Remarks}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Sec.}{Secs.}
\Crefname{subsection}{Section}{Sections}
\crefname{subsubsection}{Sec.}{Secs.}
\Crefname{subsubsection}{Section}{Sections}
\crefname{appendix}{App.}{Apps.}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Figure}{Figures}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\crefname{lstlisting}{Lst.}{Lsts.}
\Crefname{lstlisting}{Listing}{Listings}
\definecolor{ThemeOrange}{HTML}{FFA532}      \definecolor{ThemeGoldBrown}{HTML}{A98426}
\definecolor{ThemeNavy}{HTML}{0E2344}        \definecolor{ThemeBlue}{HTML}{0073CA}
\definecolor{ThemePurple}{HTML}{8A05B7}
\definecolor{ThemeGray}{HTML}{7f7f7f}        \definecolor{ThemeTeal}{HTML}{0B7285}        \definecolor{ThemeAmberText}{HTML}{C77400}   

\definecolor{BoxFormalBg}{HTML}{F4F6F9}
\definecolor{BoxFormalFrame}{HTML}{8A9BB5}
\definecolor{BoxDefBg}{HTML}{EFF5FB}
\definecolor{BoxDefFrame}{HTML}{7FAED4}
\definecolor{BoxWarmBg}{HTML}{FDF6ED}
\definecolor{BoxWarmFrame}{HTML}{C4A24D}


\newcommand{\introtakeawaybox}[2][]{\begin{tcolorbox}[colback=ThemeGoldBrown!5,
      colframe=ThemeGoldBrown!35,
      boxrule=0.6pt,
      arc=3pt,
      left=5pt, right=5pt, top=2.5pt, bottom=2.5pt,
      fontupper={\small}
  ]
    \if\relax\detokenize{#1}\relax\textbf{Contributions:} #2\else\textbf{Contributions #1:} #2\fi\end{tcolorbox}\vspace*{-0.1cm}
}

\newcommand{\takeawaybox}[2][]{\begin{tcolorbox}[
       colback=ThemeGoldBrown!5,
    colframe=ThemeGoldBrown!35,
    boxrule=0.6pt,
    arc=3pt,
    left=6pt, right=6pt, top=3.5pt, bottom=3.5pt,
    fontupper={\small}
  ]
    \IfNoValueTF{#1}{\textbf{Takeaway:} #2}{\textbf{#1} #2}\end{tcolorbox}\vspace*{-0.1cm}
}

\newcommand{\theorybox}[2][]{\begin{tcolorbox}[
       breakable,
       colback=ThemeNavy!3,
       colframe=ThemeNavy!35,
       boxrule=0.6pt,
       arc=3pt,
       left=6pt, right=6pt, top=3.5pt, bottom=3.5pt,
       fontupper={\small}
  ]
    \IfNoValueTF{#1}{\textbf{Theory summary:} #2}{\textbf{#1} #2}\end{tcolorbox}\vspace*{-0.1cm}
}

\newcommand{\empiricaltakeawaybox}[2][]{\begin{tcolorbox}[
      colback=ThemeGoldBrown!5,
    colframe=ThemeGoldBrown!35,
    boxrule=0.6pt,
    arc=3pt,
    left=6pt, right=6pt, top=3.5pt, bottom=3.5pt,
    fontupper={\small}
  ]
    \IfNoValueTF{#1}{\textbf{Empirical Takeaway:} #2}{\textbf{Empirical Takeaways #1:} #2}\end{tcolorbox}\vspace*{-0.1cm}
}

\tcolorboxenvironment{theorem}{
  enhanced, colback=ThemeNavy!3, colframe=ThemeNavy!35,
  fonttitle=\bfseries, boxrule=0.6pt, arc=3pt,
  left=6pt, right=6pt, top=3.5pt, bottom=3.5pt
}
\tcolorboxenvironment{assumption}{
  enhanced, colback=ThemeNavy!3, colframe=ThemeNavy!35,
  fonttitle=\bfseries, boxrule=0.6pt, arc=3pt,
  left=6pt, right=6pt, top=3.5pt, bottom=3.5pt
}
\tcolorboxenvironment{proposition}{
  enhanced, breakable, colback=ThemeNavy!3, colframe=ThemeNavy!35,
  fonttitle=\bfseries, boxrule=0.6pt, arc=3pt,
  left=6pt, right=6pt, top=3.5pt, bottom=3.5pt
}
\tcolorboxenvironment{definition}{
  enhanced, breakable, colback=ThemeNavy!3, colframe=ThemeNavy!35,
  fonttitle=\bfseries, boxrule=0.6pt, arc=3pt,
  left=6pt, right=6pt, top=3.5pt, bottom=3.5pt
}
\definecolor{lightwheat}{rgb}{1.0, 0.98, 0.82}
\definecolor{skyblue}{HTML}{A7C7E7}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\lstdefinestyle{pythonstyle}{
  language=Python,
  basicstyle=\ttfamily\scriptsize,
  keywordstyle=\color{blue!70!black},
  commentstyle=\color{green!50!black},
  stringstyle=\color{red!60!black},
  showstringspaces=false,
  breaklines=true,
  frame=single,
  framerule=0.4pt,
  rulecolor=\color{gray!50},
  backgroundcolor=\color{gray!3},
  columns=fullflexible,
  keepspaces=true,
}

\lstdefinelanguage{RSDiff}{
  sensitive=false,
  morecomment=[f][\color{red!60!black}]{-},
  morecomment=[f][\color{green!45!black}]{+},
  morecomment=[f][\color{ThemeNavy}]{@@},
  morecomment=[f][\color{ThemeNavy}]{diff },
  morecomment=[f][\color{ThemeNavy}]{index },
}
\lstdefinestyle{rsdiff}{
  language=RSDiff,
  basicstyle=\ttfamily\scriptsize,
  columns=fullflexible,
  keepspaces=true,
  frame=single,
  framerule=0.4pt,
  rulecolor=\color{gray!45},
  backgroundcolor=\color{white},
  breaklines=true,
  postbreak=\mbox{\textcolor{gray}{$\hookrightarrow$}\space},
  xleftmargin=1em,
  xrightmargin=1em,
  aboveskip=0.5em,
  belowskip=0.5em,
}
\newtcolorbox{promptbox}[2][]{breakable, enhanced,
  colback=white, colframe=ThemeNavy!70,
  boxrule=0.5pt, arc=2pt,
  left=6pt, right=6pt, top=4pt, bottom=4pt,
  fonttitle=\bfseries\small, coltitle=white,
  colbacktitle=ThemeNavy!70,
  title={#2}, #1
}
\DefineVerbatimEnvironment{PromptVerb}{Verbatim}{breaklines=true, fontsize=\scriptsize,
  breaksymbolleft={\textcolor{gray}{\scriptsize$\hookrightarrow$}}}

\newcommand{\slotnum}[1]{\textcolor{ThemeBlue}{$\mathbf{#1}$}}
\newcommand{\noslot}{\textcolor{ThemeGray}{$\varnothing$}}



\newcommand{\ourmethod}{\texttt{RQGM}\xspace}
\newcommand{\theourmethod}{the \ourmethod}
\newcommand{\Theourmethod}{The \ourmethod}
\newcommand{\AI}{\texttt{AI}}
\newcommand{\hgm}{\texttt{HGM}\xspace}
\newcommand{\hgmh}{\texttt{HGM-H}\xspace}
\newcommand{\dgm}{\texttt{DGM}\xspace}
\newcommand{\dgmh}{\texttt{DGM-H}\xspace}
\newcommand{\hyperagents}{\texttt{HyperAgents}\xspace}
\newcommand{\proofautograder}{\texttt{ProofAutoGrader}\xspace}
\newcommand{\sakana}{\texttt{Sakana}\xspace}
\newcommand{\imocode}{\texttt{IMO25}\xspace}
\newcommand{\gptlow}{\texttt{GPT-5.5}\xspace}
\newcommand{\nemotron}{\texttt{Nemotron} \texttt{3} \texttt{Super}\xspace}
\newcommand{\nemotronultra}{\texttt{Nemotron} \texttt{3} \texttt{Ultra}\xspace}
\newcommand{\astra}{\texttt{GPT-6} \texttt{Astra}\xspace}
\newcommand{\cmp}{\texttt{CMP}\xspace}
\newcommand{\apres}{\texttt{APReS}\xspace}
\newcommand{\polyglot}{\texttt{Polyglot}\xspace}
\newcommand{\crave}{\texttt{CRAVE}\xspace}
\newcommand{\deepswe}{\texttt{DeepSWE}\xspace}
\newcommand{\imogradbench}{\texttt{IMO-GradingBench}\xspace}
\newcommand{\swebench}{\texttt{SWE-bench}\xspace}
\definecolor{RedQueenRed}{HTML}{B01030}
\newcommand{\redqueencrownedheart}{\raisebox{-0.08em}{\smash{\begin{tikzpicture}[x=0.045em,y=-0.045em,baseline=-0.45ex]
      \path[fill=RedQueenRed,draw=none]
        (0,11)
        .. controls (-7.5,4) and (-12,-0.5) .. (-12,-5)
        .. controls (-12,-9) and (-8.8,-11) .. (-5.6,-11)
        .. controls (-2.6,-11) and (-0.8,-9) .. (0,-7)
        .. controls (0.8,-9) and (2.6,-11) .. (5.6,-11)
        .. controls (8.8,-11) and (12,-9) .. (12,-5)
        .. controls (12,-0.5) and (7.5,4) .. (0,11)
        -- cycle;
      \path[fill=RedQueenRed,draw=none]
        (-7,-9) -- (-7,-13.6) -- (-3.4,-10.8) -- (0,-16)
        -- (3.4,-10.8) -- (7,-13.6) -- (7,-9) -- cycle;
    \end{tikzpicture}}}}

\newcommand{\redqueenmark}{\begin{tikzpicture}[x=0.18em,y=-0.18em,baseline=-0.5ex]
    \path[fill=RedQueenRed,draw=RedQueenRed!75!black,line width=0.2pt]
      (0,11)
      .. controls (-7.5,4) and (-12,-0.5) .. (-12,-5)
      .. controls (-12,-9) and (-8.8,-11) .. (-5.6,-11)
      .. controls (-2.6,-11) and (-0.8,-9) .. (0,-7)
      .. controls (0.8,-9) and (2.6,-11) .. (5.6,-11)
      .. controls (8.8,-11) and (12,-9) .. (12,-5)
      .. controls (12,-0.5) and (7.5,4) .. (0,11)
      -- cycle;
    \path[fill=RedQueenRed!85!black,draw=none]
      (-7,-9) -- (-7,-13.6) -- (-3.4,-10.8) -- (0,-16)
      -- (3.4,-10.8) -- (7,-13.6) -- (7,-9) -- cycle;
  \end{tikzpicture}}

\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}

\newcommand{\func}[1]{\mathrm{#1}}

\makeatother


==> preamble/packages.tex <==
\makeatletter

\RequirePackage{etoolbox}   
\RequirePackage{iftex}
\ifpapericlr
  \RequirePackage[T1]{fontenc}
  \RequirePackage{times}
\else
\ifPDFTeX
  \RequirePackage[utf8]{inputenc}
  \RequirePackage[T1]{fontenc}
  \RequirePackage{tgtermes}
  \RequirePackage[matchlowercase]{tgheros}
  \RequirePackage[matchlowercase]{tgcursor}
\else
  \RequirePackage{fontspec}
  \defaultfontfeatures{Ligatures=TeX}
  \setmainfont[
    BoldFont=texgyretermes-bold.otf,
    ItalicFont=texgyretermes-italic.otf,
    BoldItalicFont=texgyretermes-bolditalic.otf
  ]{texgyretermes-regular.otf}
  \setsansfont[
    BoldFont=texgyreheros-bold.otf,
    ItalicFont=texgyreheros-italic.otf,
    BoldItalicFont=texgyreheros-bolditalic.otf,
    Scale=MatchLowercase
  ]{texgyreheros-regular.otf}
  \setmonofont[
    BoldFont=texgyrecursor-bold.otf,
    ItalicFont=texgyrecursor-italic.otf,
    BoldItalicFont=texgyrecursor-bolditalic.otf,
    Scale=MatchLowercase
  ]{texgyrecursor-regular.otf}
\fi

\fi

\PassOptionsToPackage{table}{xcolor}
\RequirePackage{graphicx}
\RequirePackage{booktabs}        \RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsfonts}
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{microtype}
\ifpapericlr
  \microtypesetup{expansion=false,protrusion=false}
\else
\ifPDFTeX
  \microtypesetup{activate={true,nocompatibility},final,expansion=true,protrusion=true,factor=1100,stretch=20,shrink=20}
  \DisableLigatures{encoding=T1,family=tt*}
\else
  \microtypesetup{activate={true,nocompatibility},final,expansion=false,protrusion=true,factor=1100}
\fi
\fi
\frenchspacing
\RequirePackage{xcolor}
\RequirePackage{nicefrac}
\RequirePackage{xspace}
\RequirePackage{xparse}
\RequirePackage{url}
\ifpapericlr\RequirePackage{xurl}\fi
\RequirePackage{float}
\RequirePackage{wrapfig}
\ifpapericlr
  \RenewDocumentEnvironment{wrapfigure}{o m o m}{\begin{figure}[tbp]\centering\begin{minipage}{#4}}{\end{minipage}\end{figure}}
\fi
\RequirePackage{placeins}
\RequirePackage{enumitem}
\RequirePackage{tabularx}
\RequirePackage{multirow}
\RequirePackage{colortbl}
\RequirePackage{listings}
\RequirePackage{fvextra}  \RequirePackage{stmaryrd}
\RequirePackage{newtxmath}  \RequirePackage{bm}
\def\fontsubfuzz{.6pt}
\RequirePackage{caption}
\RequirePackage[skins,breakable,theorems]{tcolorbox}
\RequirePackage{siunitx}\sisetup{round-mode=places, round-precision=2}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,positioning,shapes.geometric,calc,fit,backgrounds}
\RequirePackage{subcaption}      \RequirePackage{etoc}            \ifpaper@mlsys
  \let\algorithm\relax
  \let\endalgorithm\relax
  \let\listofalgorithms\relax
  \expandafter\let\csname algorithm*\endcsname\relax
  \expandafter\let\csname endalgorithm*\endcsname\relax
\fi
\RequirePackage[ruled,vlined]{algorithm2e}

\RequirePackage[toc, title]{appendix}

\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\definecolor{paperlink}{rgb}{0.10,0.20,0.55}
\hypersetup{colorlinks=true, linkcolor=paperlink, citecolor=paperlink, urlcolor=paperlink, breaklinks=true}
\RequirePackage[capitalise, nameinlink]{cleveref}

\makeatother

